GMP-AR: Granularity Message Passing and Adaptive Reconciliation for Temporal Hierarchy Forecasting

Time series forecasts of different temporal granularity are widely used in real-world applications, e.g., sales prediction in days and weeks for making different inventory plans. However, these tasks are usually solved separately without ensuring coherence, which is crucial for aligning downstream decisions. Previous works mainly focus on ensuring coherence with some straightforward methods, e.g., aggregation from the forecasts of fine granularity to the coarse ones, and allocation from the coarse granularity to the fine ones. These methods merely take the temporal hierarchical structure to maintain coherence without improving the forecasting accuracy. In this paper, we propose a novel granularity message-passing mechanism (GMP) that leverages temporal hierarchy information to improve forecasting performance and also utilizes an adaptive reconciliation (AR) strategy to maintain coherence without performance loss. Furthermore, we introduce an optimization module to achieve task-based targets while adhering to more real-world constraints. Experiments on real-world datasets demonstrate that our framework (GMP-AR) achieves superior performances on temporal hierarchical forecasting tasks compared to state-of-the-art methods. In addition, our framework has been successfully applied to a real-world task of payment traffic management in Alipay by integrating with the task-based optimization module.

==> latex/abstract.tex <==
Time series forecasts of different temporal granularity are widely used in real-world applications, e.g., sales prediction in days and weeks for making different inventory plans. However, these tasks are usually solved separately without ensuring coherence, which is crucial for aligning downstream decisions. Previous works mainly focus on ensuring coherence with some straightforward methods, e.g., aggregation from the forecasts of fine granularity to the coarse ones, and allocation from the coarse granularity to the fine ones. These methods merely take the temporal hierarchical structure to maintain coherence without improving the forecasting accuracy. In this paper, we propose a novel granularity message-passing mechanism (GMP) that leverages temporal hierarchy information to improve forecasting performance and also utilizes an adaptive reconciliation (AR) strategy to maintain coherence without performance loss. Furthermore, we introduce an optimization module to achieve task-based targets while adhering to more real-world constraints. Experiments on real-world datasets demonstrate that our framework (GMP-AR) achieves superior performances on temporal hierarchical forecasting tasks compared to state-of-the-art methods. In addition, our framework has been successfully applied to a real-world task of payment traffic management in Alipay\footnote{www.alipay.com} by integrating with the task-based optimization module.
% Our framework can seamlessly integrate with the optimization module to address real-world tasks, as demonstrated by its successful application in AliPay's payment traffic management.
% Our framework combined with the optimization module can be applied to real-world tasks effectively without any additional effort under the coherence constraint.
% Our neural-weighted methods can be applied to real-world tasks effectively without any additional effort under the coherence constraint.

==> latex/backgrounds.tex <==
% \section{Preliminaries}
% \label{section: preliminaries}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/thier.png}
%     \caption{The notation of each node in figure \ref{fig:temporal_hts} at time point $\tau  =0$}
%     \label{fig:temporal_hier}
% \end{figure}

 In this section, we provide background on temporal hierarchical time series and introduce necessary notations here for ease of understanding.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/hier_structure_notation_v2.png}
    \caption{The notation of each node in Fig.~\ref{fig:temporal_hts} observed at timestamp $t = 6$ and $\tau  = 1$.}
    \label{fig:temporal_hier}
    \vspace{-5mm}
\end{figure}

\subsection{Preliminaries: Temporary Hierarchical Structure}
The time series is denoted by $\{y_t; 1 \le t \le T\}$ with a fixed sampling frequency ({\it base frequency}), which is of the finest granularity. The time series of the coarser granularity is aggregated by non-overlapping and regularly sampled values $y_t$ as Eq.~\eqref{agg_expression} shows. For the time series in Fig. \ref{fig:temporal_hts}, the base frequency is ten-minute. It is aggregated into a half-hour value with three ten-minute sample values, and an hourly frequency with two half-hour sample values.

The temporal HTS can be expressed as a tree structure with a linear aggregation constraint called \textit{coherence constraint}, formulated via an aggregation matrix $\mathbf{S}\in \mathbb{R}^{n \times m}$ (see Eq.~\eqref{eq_sum}), where $m = 6$ is the number of leaf nodes and $n = 9$ is the total number of nodes in the tree in Fig.~\ref{fig:temporal_hts}.
 
We consider a \textit{p-level} aggregated temporal hierarchical structure. The number of nodes at each level can be presented as $N_p = \{n_k: k  = 1, 2, \dots, p \}$, where $n_1 = 1$, and $n_p = m$. Take Fig.~\ref{fig:temporal_hts} as an example, $N_3 = \{1, 2, 6\}$. The sample values at timestamps in the time series at level $k$ can be expressed as

\begin{equation}
\label{agg_expression}
    y_{(\tau - 1)n_k+j}^{[k]} = \sum_{t=(\tau-1) m +(j-1)m_k+1} ^ {(\tau-1) m+jm_k} y_t, \,1\le j \le n_k,
\end{equation}
where $\tau \in \{1,\dots, \lfloor\frac{T}{m}\rfloor\}$ is the observation index of the
most aggregated time series (i.e., the one at the root level), and $j$ is the observation index at level $k$ in the temporal structure, and $m_k = \frac{m}{n_k}$ is the number of leaves aggregated to generate the node values at the $k$-th level. One can see that the values $\{\displaystyle{y^{[k]}_{\tau n_k}},1\le k \le p\}$ are observed at the same time point $\tau m$.
% as well as which also means the children number on the level. 

In the temporal hierarchical structure, the leaf nodes are called the \textit{bottom-level} series: $\by^{[p]}_{\tau}\in \mathbb{R}^{m}$, and the remaining nodes are termed \textit{upper-levels} series: $\{y^{[1]}_{\tau}, \dots, \by^{[p-1]}_{\tau} \}$.  The number of nodes at upper levels is $r=\sum_{i=1}^{p-1} n_i$.
Obviously, the total number of nodes $n=r+m$, and $\by_{\tau} :=[y^{[1]}_{\tau}, {\by^{[2]}_{\tau}}^{\mathsf{T}}, \dots, {\by^{[p]}_{\tau}}^{\mathsf{T}}]^{\mathsf{T}} \in  \mathbb{R}^{n} $ contains observations at time $\tau $ for all levels, which satisfies  
\begin{equation}
\label{eq_sum}
\by_{\tau }=\bS \by^{[p]}_{\tau },
\end{equation}
% at time step $t$.
where $\bS\in \{0,1\}^{n \times m}$ is an aggregation matrix. 

Taking Fig.~\ref{fig:temporal_hts} as an example, the aggregation matrix 
% \replace{takes}
is
% as in Eq.~\eqref{eq:hts_matrix}

\begin{equation*} %\label{eq:hts_matrix}
    \bS = 
    \begin{pmatrix}
        \bS_{\text{sum}}\\
        \mathbf{I}_6
    \end{pmatrix}
    =
    \begin{pmatrix}
    \begin{array}{cccccc}
        1 & 1 & 1 &1 & 1 &1 \\
        1 & 1 & 1 &0 &0 &0\\
        0 & 0 & 0 &1 &1 & 1\\
        % \hline \\
        \hdotsfor{6}\\
        % & & & & \\
        & & \mathbf{I}_6 & &\\
        % & & & &
     \end{array} 
     \end{pmatrix}
     % \right]
     ,
\end{equation*}
% Figure ~\ref{fig:hier_timeseries}, 
the total number of nodes in the hierarchy is $n=1+2+6$, and the number of notes at upper-levels is $r=3$.  At each time index $\tau$, 
% \begin{equation*}
%     \begin{aligned}
%         \mathbf{u}_{t}&=[y_{A,t},y_{B,t},y_{C,t}] \in \mathbb{R}^{3}, \\
%         \mathbf{b}_{t}&=[y_{D,t},y_{E,t},y_{F,t},y_{G,t},y_{H,t}] \in \mathbb{R}^{5},\\
%         y_{A,t}&=y_{B,t}+y_{C,t}=y_{D,t}+y_{E,t}+y_{F,t}+y_{G,t}+y_{H,t}.
%     \end{aligned}
% \end{equation*}
% $ and $\mathbf{b}_{t}=[y_{D,t},y_{E,t},y_{F,t},y_{G,t},y_{H,t}] \in \mathbb{R}^{5}$, $y_{A,t}=y_{B,t}+y_{C,t}=y_{D,t}+y_{E,t}+y_{F,t}+y_{G,t}+y_{H,t} $.
% , and the aggregation matrix $\bS\in \{0,1\}^{8 \times 5}$.
the coherence constraint of Eq.~\eqref{eq_sum} can be represented as ~\cite{rangapuram2021end}
\begin{equation}
\label{eq:coherent_co}
\mathbf{A}\by_{\tau}=\mathbf{0},
\end{equation}
where $\mathbf{A}:=\left (\mathbf{I}_{r}|-\bS_{\text{sum}}\right ) \in \{0,1\}^{r \times n}$, $\mathbf{0}\in \mathbb{R}^r$ is the zero vector, and $\mathbf{I}_{r} \in \mathbb{R}^{r \times r}$ is the identity matrix.  %We will use this formula as the coherence constraint for the rest of the paper.

\subsection{Related Work} 

\subsubsection{HTS Forecasting.}
% The most well-addressed hierarchical structure in the field of time series forecasting is tree structure in the cross-sectional dimension of multivariate time series, 
Multivariate hierarchical time series is more well-addressed than temporal HTS where each node in the hierarchy represents an individual time series~\cite{Hyndman2011Optimal,taieb2017coherent, corani2020probabilistic}.
Most previous methods~(\cite{han2021simultaneously, das2022deep}) follow a two-stage approach that traditional statistical and deep learning forecasting methods are used to generate the base forecasts followed by a reconciliation step to ensure that the base forecasts are coherent. 
% However, \replace{due to the superior performance of deep neural networks,}{deep learning methods have shown superior performance to traditional statistical methods for forecasting univariate time series.} \replace{deep-learning forecasting}{Deep learning} methods such as DeepAR~\cite{salinas2020deepar} and DeepVAR~\cite{salinas2019high} have been developed. 
However, these forecasting methods do not leverage the hierarchy structure to improve the forecasting performance except ~\cite{SLOTH_2023}
that does explicitly utilize the hierarchy information. 
However, SLOTH ignores the temporal information in the temporal hierarchy and the bottom-up attention mechanism is too complex and time-consuming. 
As for the reconciliation method, traditional approaches depend on the forecast of one level, such as bottom-up~\cite{gross1990disaggregation}, top down~\cite{athanasopoulos2009hierarchical}. However, these methods only employ single-level forecasts to conduct reconciliation ignoring the forecasts of other levels. 
The MinT~\cite{wickramasuriya2019optimal} leverages all level information of base distribution forecasts to generate coherent results based on the unbiased forecasting assumption, which limits its applicability and performance in real-world scenarios.
The closed-form projection {approach}~\cite{rangapuram2021end} achieves an end-to-end reconciliation without any assumption, but the adjustments to the base forecast are unreasonable sometimes, such as large adjustments for nodes with small values and small adjustments for nodes with large values that cause forecasting performance loss.

\subsubsection{Temporal Hierarchical Forecasting.} 
% The core concept of \textit{temporal hierarchical forecasting} for time series is defined in~\cite{thts_2017, theodosiou2021forecasting}, 
% where traditional statistical multivariate HTS methods are employed.  
The temporal hierarchical forecasting defined in~\cite{thts_2017} requires coherence constraint among temporal granularity,
and forecasting tourism data with coherence on both cross-sectional and temporal dimensions is studied in~\cite{Kourentzes2019Cross}. They rely on statistical tools for the reconciliation of base forecasts. \cite{multiscale_rnn21} is also aimed at improving the forecasting accuracy of time series with different levels of granularity. However, this work does not address coherence. 
Recently, an end-to-end model (COPDeepAR) is proposed in~\cite{rangapuram2023} that focuses on generating coherent probabilistic forecasts for time series with various levels of granularity. This is achieved by utilizing GNNs to extract inter-level information and applying a closed-form projection reconciliation method to maintain coherence. 
% Although GNNs are a common tool for extracting information from structured data, temporal hierarchy is actually a tree structure. 
GNNs introduce spurious connections among all nodes but valid information actually only exists between parent and child nodes. Therefore, it fails to capture structure information because of noise connections and results in loss of forecasting performance as pointed out in \cite{SLOTH_2023}. In our works, we propose a more efficient information extraction mechanism between different granularity in the temporal hierarchy.


 





==> latex/conclusion.tex <==
In this paper, we introduced a novel structure-learning framework for temporal hierarchical time series (GMP-AR).
% \replace{, with a granularity message-passing mechanism incorporating the temporal and hierarchical information}
{Our framework incorporated temporal and hierarchical information with a message passing mechanism} to improve the performance of base forecasts, which is
% \replace{, where the granularity input transformation module focuses on enriching the information of temporal input of each node and our two granularity feature fusion modules focus on integrating the temporal and hierarchical features.}
{consisted of several modules, i.e., the granularity input transformation module that enriches the information of the temporal input of each node and the other two granularity feature fusion modules integrating the temporal and hierarchical features. }
% The adaptive reconciliation method keeps coherence without any loss in forecasting performance. It uses a node-dependent weighted optimization target to precisely control the adjustment scale for each node.
For reconciliation, we proposed an adaptive reconciliation method to ensure coherence without any loss in forecasting performance by utilizing the node-dependent weighted optimization target to precisely control the adjustment scale for each node. 
We also provided a `plug-and-play' optimization module that incorporates task-based targets and realistic constraints to solve real-world temporal HTS problems.  
We conducted extensive empirical evaluations on real-world datasets to validate our method, demonstrating the competitiveness of our approach compared with other state-of-the-art methods. Furthermore, our ablation studies verify the efficacy of each designed component.
Our framework combining with the optimization module has been applied in the payment traffic management system in Alipay successfully.

==> latex/experiment.tex <==
In this section, we empirically evaluate our proposed method on public time series datasets (details are in Appendix B) and 
% The time granularity ranges from 1 hour to 5 days.  
% We first compare our method to three baselines: 1)traditional statistical temporal hierarchical baselines in Thief~\cite{thts_2017}, 2). representative deep learning models with popular reconciliation on forecasting performance and 3). traditional HTS method. The details of baselines are provided in Appendix C.  
representative SOTA methods (details are shown in Appendix C).
We then present the successful application of our method with the task-based optimization module in the real-world payment traffic management system of Alipay.  The experiment setup is described in Appendix G and the implementation code is included in the supplementary files.


\newcolumntype{s}{>{\hsize=1.2\hsize}X}
% \newcolumntype{s}{>{\hsize=12.0\hsize\normal}X}
% \setlength{\tabcolsep}{2pt}
\begin{table*}[t]
    \centering
    \small
    \resizebox{0.85\textwidth}{!}
    {
    % \begin{tabularx}{\textwidth}{s|cc|cc|cc}
    \begin{tabularx}{\textwidth}{l|cc|cc|cc}
        \hline
         \textbf{Dataset} & \multicolumn{2}{c}{Electricity}  & \multicolumn{2}{c}{Traffic} & \multicolumn{2}{c}{Exchange Rate}  \\ \hline
         \textbf{Metrics} & b-MAPE & MAPE & b-MAPE& MAPE & b-MAPE & MAPE  \\ \hline
         % ARIMA-BU & 0.000(0.000)& 0.000(0.000)& 0.000(0.000)& 0.000(0.000) & 0.000(0.000)& 0.000(0.000) & 0.000(0.000)& 0.000(0.000) \\ 
         % ARIMA-MINT-SHR & & & & & & & & \\ \hline
         THIEF-ARIMA-BU &0.1895 & \textbf{0.1319} & 0.7501 & 0.5518 &  0.0095 & 0.0092\\ 
         THIEF-ETS-BU  &0.3712 &  0.3111 & 0.8815&  0.8600 &0.0100 & 
        0.0096)\\
         THIEF-THETA-BU  & 0.2071 &  0.1434 & 0.7064 & 0.7065 & 0.0102&   0.0099\\
         THIEF-ARIMA-OLS  & 0.1896 & 0.1319& 0.8293 & 0.5711 &  0.0118 & 0.0113\\
         THIEF-ETS-OLS  & 0.2208& 0.1438 & 1.0477 & 0.6871 & 0.0133& 0.0102 \\ 
         THIEF-THETA-OLS  &0.2256 & 0.1520 & 1.6886& 0.8952 & 0.0099 & 0.0094 \\
         THIEF-ARIMA-MSE  & 0.1906 & 0.1333 &  0.7000 & 0.5141 & 0.0097 & 0.0093\\
         THIEF-ETS-MSE  &0.2142 &  0.1473& 0.7315& 0.6872& 0.0103& 0.0100\\
         THIEF-THETA-MSE  & 0.2036 & 0.1373 &  0.9467 &  0.7035 & 0.0094& 0.0090\\ \hline
         % THIEF-ARIMA-STRUCT  & & & & & & & & \\
         % THIEF-ETS-STRUCT  & & & & & & & & \\ \hline
         % DeepAR-BU & 0.3573(0.0368) & 0.3507(0.0387) & 1.2647(0.3643) & 0.7542(0.1841) & 0.012(0.0011) & 0.0117(0.0011) & & \\ 
         % NBeats-BU & 0.2514(0.0245) & 0.2947(0.0268) & 0.8795(0.114) & 0.6353(0.0477) &0.145(0.0551) & 0.1212(0.0687) & & \\ 
         % Autoformer-BU & 0.4324(0.0795) & 0.4395(0.0549) & 1.3449(0.3393) & 0.8086(0.1592) &0.0199(0.0101) &0.019(0.0101) & & \\ 
         DeepAR-BU & 0.4168(0.0182) & 0.4210(0.0154) &1.3439(0.0172) & 0.8885(0.0219) & 0.0138(0.0027) &  0.0136(0.0030) \\ 
         NBeats-BU & 0.2683(0.0383)& 0.3000(0.0318) & 0.5601(0.0570)& 0.4292(0.0377)&0.0196(0.0062)& 0.0192(0.0064)\\ 
         Autoformer-BU & 0.4059(0.1022) & 0.4049(0.0859) & 1.6798(0.2757) & 0.9505(0.1362)&0.0092(0.0006) &0.0087(0.0006) \\
         DeepAR-Proj & 0.4167(0.0042) & 0.3889(0.0023) & 3.3717(0.0290) &1.6043(0.0138) & 0.0114(0.0019) & 0.0111(0.0019)\\ 
         NBeats-Proj & 0.2432(0.0173)& 0.2799(0.0203) & 0.7422(0.0676) & 0.5308(0.0297) &0.0211(0.0072) & 0.0207(0.0075)\\ 
         Autoformer-Proj &0.2754(0.0047) & 0.3024(0.0064) & 1.1376(0.0758)& 0.6768(0.0382) & 0.0111(0.0007) & 0.0107(0.0007)\\ 
         DeepAR-TDProb & 0.1761(0.0055) & 0.2370(0.0035) & 1.0536(0.0296) &  0.6455(0.0126) & 0.0096(0.0008) & 0.0094(0.0008) \\ 
         NBeats-TDProb &0.1830(0.0081) & 0.2395(0.0098) & 1.0744(0.0339)&0.6662(0.0142) &0.0161(0.0060) & 0.0159(0.0061)\\ 
         Autoformer-TDProb & 0.2052(0.0243) & 0.2704(0.0268) & 0.9894(0.0395)& 0.6244(0.0198) & 0.0120(0.0035) &0.0118(0.0035)  \\ \hline
         HierE2E & 0.2346(0.0148) & 0.2980(0.0139)& 0.4728(0.0180) & 0.4768(0.0128) & 0.0145(0.0017) & 0.0136(0.0016)\\ 
         SHARQ & 0.2101(0.0058) & 0.2730(0.0051) &0.5041(0.0086) & 0.5041(0.0128) & 0.0156(0.0043)& 0.0138(0.0033)\\ 
         COPDeepAR &  0.6088(0.0531) & 0.7309(0.0542) & 0.8345(0.0058)& 0.8202(0.0060) & 0.1247(0.0274)& 0.1246(0.0275) \\
         SLOTH &  0.1765(0.0022)& 0.2424(0.0027) & 0.4621(0.0026)& 0.4616(0.0019) & 0.0114(0.0003)& 0.0110(0.0003)
         \\ \hline
         
         GMP-BU &0.1711(0.0074) & 0.2288(0.0079) & 0.4484(0.021) & 0.3932(0.0145)& 0.0107(0.0014)& 0.0102(0.0015) \\ 
         GMP-TDProb & 0.1731(0.0026) & 0.2331(0.0044) & 0.9989(0.0301) & 0.6047(0.0112)& 0.0088(0.0009)& 0.0085(0.0009)\\ 
         GMP-Proj &0.1937(0.0143) & 0.2481(0.0131) & 0.4868(0.0243) & 0.4083(0.0094)  &0.0089(0.0024) & 0.0086(0.0025) \\ 
         GMP-AR & \textbf{0.1499(0.0021)} & 0.2158(0.003) & \textbf{0.4289(0.0202)}& \textbf{0.3798(0.0066)} &\textbf{0.0085(0.0021)} & \textbf{0.0082(0.0021)}\\ \hline
         % THTS-Optimize & & & & & & & & \\ 
    \end{tabularx}
    }
    \caption{B-MAPE (bottom MAPE) and MAPE metric values over five independent runs for baselines such as traditional reconciliation methods, deep learning methods, and popular multivariate HTS methods,  as well as our approach. The values in brackets are the variances over five runs.}
    \label{tab:result}
    \vspace{-5mm}
\end{table*}


\subsection{Result Analysis}
% metrics 
In this section, we {evaluate} the {forecasting} performance of our proposed method on three public datasets.  We use the mean absolute percentage error to measure the performance of each method, both at the bottom level (b-MAPE) that has the finest granularity and across all nodes (MAPE).

The experimental results are {shown} in Table~\ref{tab:result}.  The top section shows the results of the traditional statistic method, Thief; The second section {shows} results from deep neural networks methods with bottom-up (BU),  closed-formed projection (Proj)~\cite{rangapuram2021end} and top down proportion (TDProb)~\cite{das2022deep} reconciliation; The third section {shows the results of} popular multivariate hierarchical time series forecasting methods (HierE2E, SHARQ, COPDeepAR, SLOTH); The bottom section {shows the results of} our forecasting approach (GMP) and the combination of our forecasting mechanism with popular reconciliation methods (BU, Proj, TDProb), as well as our adaptive reconciliation with weighted projection (AR) method.

For the bottom-level metrics (b-MAPE), DeepAR~\cite{salinas2020deepar} with TDProb reconciliation performs the best on the Electricity and Exchange Rate datasets, and NBeats with BU reconciliation performs the best on the Traffic datasets. In general, the performance of statistical methods in Thief is more stable {than the} deep learning models, but deep models achieve the best performances across all baselines. 
One can observe that models of best performance on b-MAPE do not necessarily perform as well on MAPE, which is caused by different level contributions to the overall performance. For example,  the temporal patterns and scales of different levels can be diverse.
For overall metrics, statistic methods in Thief outperform other baselines and our methods on Electricity datasets, and multivariate HTS methods have superior performance than deep learning methods. This  because HTS methods take all nodes into consideration while modeling.

Our proposed approach, GMP-AR, delivers an average performance increase of over $2\% \sim 3\%$ compared to other methods on both b-MAPE and MAPE metrics in most scenarios on the Electricity and Traffic datasets. Specifically, GMP with AR Projection achieves the best performance for b-MAPE among all models on all three datasets, and it also performs the best on MAPE on Traffic and Exchange Rate datasets.
In addition to adaptive reconciliation, we also combine our forecasting mechanism (GMP) with the aforementioned popular reconciliation methods (BU, Proj TDProb). These combinations also achieve higher accuracy than the baselines.  
We also assess the performance across all levels (Appendix D) and running time (Appendix E), and the ablation study for each component in the GMP forecasting framework (Appendix F). 

In conclusion, our GMP-AR mechanism achieves the best forecasting accuracy by utilizing both temporal and granularity hierarchical information. The adaptive reconciliation produces coherent results while also improving the forecasting performance.

\subsection{Alipay Payment Traffic Management}
Alipay is a world-leading third-party online payment service platform that provides billions of users with online and mobile payment services. These services support amount to billions of transactions and trillions of dollars daily, which has been widely recognized as a significant contribution to the orderly development and digital upgrading of society and economy. To ensure a stable and reliable payment experience for users, it is necessary to forecast future payment traffic in advance to ensure that the massive {number} of payment transactions and amounts can be effectively supported at the infrastructure and operational levels. 
% The daily payment traffic forms a natural hierarchy as Fig.~\ref{fig:alipay} shows, with total payment volume being divided into offline consumption (shopping in physical stores), online consumption (shopping on Taobao, etc.), and personal transfers, and each scenario can be further divided into the volume of various payment tools such as bank cards, Huabei, and Alipay balance. 
% Considering the complexity of the underlying technological architecture behind payment services, accurate forecast of fine-grained payment volume is necessary.  Additionally, it is also imperative to meet the traffic estimates at each level of temporal hierarchy.
In the temporal dimension, the manager needs to reschedule the underlying system resource under different granularity, i.e., hourly, daily, and longer-term like weekly. This way could help the system to support billions of payments efficiently and energy-savingly. Therefore, it is necessary to forecast payment traffic at hourly, daily, and multi-day granularity. This creates a natural three-level tree structure (see Fig.~\ref{fig:alipay}). In {this} temporal hierarchical structure, the coherence of different granularity forecasts needs to be satisfied.


\begin{figure}[t]
    \centering
    \includegraphics[width=1.\linewidth]{figures/alipay_v2.png}
    \caption{The temporal hierarchical structure of mobile payment service of Alipay, with weekly traffic forecast as the root node, daily forecast as the second level, and hourly forecast as leaf nodes ($N_3 = \{1, 7, 168\}).$}
    \label{fig:alipay}
    \vspace{-5mm}
\end{figure}
The real-world task of hierarchical time series (HTS) forecasting differs from theoretical temporal HTS forecasting for its more task-based targets and realistic constraints, which are listed as follows: 1) Target - not only must forecast accuracy be considered but also the trend of the forecast, which is vital for business corporations that interact with external banks. 2) Constraint - the root node, i.e., the base daily forecast, cannot be altered due to the historical requirements of the regulatory authority. 3) Constraint - the child nodes, i.e., the scale of adjustment must not be more than 20 percent due to the risk regulations set by the authority.  These requirements can be formulated as  % Eq.~\eqref{eq:alipay} shows:
\begin{equation}
    \label{eq:alipay}
    \begin{aligned}
      \mathcal{J}(\hat{\by}) & = \mathop{\arg\min}_{\by}{\|\hat{\by} - \by\|_2 + \beta\left(1 -\frac{\hat{\by} \by}{\|\hat{\by}\| \|\by\|} \right)}\\
    \text{s.t.}\quad &
    \begin{cases}
    \mathbf{A}\by = \mathbf{0}, \\
    \by[0] -\hat{\by}[0]= 0,\\
    abs(\by -\hat{\by}) - 0.2\hat{\by} \le \mathbf{0} ,
    \end{cases}
     \end{aligned}
\end{equation}
where we append cosine similarity with a hyperparameter multiplier $\beta$ to optimization targets to improve trend forecasting performance, and also take additional two real-world constraints into consideration.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/alipay_result.png}
    \caption{Results of five independent runs on Alipay scenarios of three methods, i.e., DeepAR (online baseline), GMP-AR, and GMP-AR with optimization module (lower MAPE and higher trend accuracy are better). Our GMP-AR with optimization module improves MAPE by 3.8\% over baselines without performance loss on trend accuracy.}
    \label{fig:alipay_result}
    \vspace{-6mm}
\end{figure}

% As shown in Figure~\ref{fig:inv_uni}, the prediction Net model performs the best on prediction (MAPE), which is the training objective.  As for the task cost, which the scheduler really cares in practice, our SLOTH framework outperforms the Prediction Net by a large margin. Specifically, our model improves the task-cost performance by 36.8\% compared to the Prediction Net, while at the same time achieving a similar task loss target as the Weighted Loss Net, but with an improvement of 53.2\% in the prediction accuracy. 

{The results} in Fig.~\ref{fig:alipay_result} show that vanilla GMP-AR performs the best on prediction accuracy by 5\%-7\% without considering trend targets and the other two task-based constraints compared to the online baseline model, DeepAR. However, the trend accuracy is lower by 5\%. Our GMP-AR combined with the optimization module achieves 3\%-5\% improvements on MAPE and remains similar trend accuracy as the baseline. {In} other words, this method achieves a compromise between forecast and trend accuracy. Besides, the results of the optimization module adhere to all task-based constraints, while vanilla GMP-AR only satisfies the coherence constraint. 

==> latex/introduction.tex <==
Time series forecasting is widely used in many important real-world tasks, such as supply chains management~\cite{athanasopoulos2009hierarchical, demandforecast13}, traffic flow prediction~\cite{traffic2017,li2018diffusion}.
Forecasting of different temporal granularity is essential for informed decision-making in downstream tasks. In management and operational scenarios, forecasting at different time scales is necessary to formulate plans that span from short-term to long-term. For instance, in the retail sales industry, managers need to make decisions about how much inventory to order and how to allocate it to different stores. Daily predictions can be used to plan the daily commodity distribution to each store, while weekly predictions can be used to purchase commodities in bulk. This ensures that the stores have the proper amount of inventory on hand to meet customer demand, while also minimizing the cost of carrying excess inventory.


As shown in Fig.~\ref{fig:temporal_hts}, a temporal hierarchical structure is formed naturally with different levels of temporal granularity. The time series of the finest granularity makes up the bottom level, and it is aggregated into upper levels of coarser granularity. This type of time series is commonly referred to as a  \textit{temporal hierarchical time series} or temporal HTS ~\cite{thts_2017}.
Temporal HTS forecasting tasks are challenging because they require accurate prediction results for different granularity while satisfying aggregation (coherence) constraints that time series at upper levels are the aggregation of those at lower levels. 
It is difficult to produce accurate predictions for all levels with a single model because time series at each level have different granularity and exhibit their own specific dynamics, such as different trends and various seasonalities.
In addition, independent forecasts (i.e., \textit{base forecasts}) are unlikely to adhere to the coherence constraints across temporal granularity. 
The inaccurate and incoherent forecasts would result in inefficient planning of downstream tasks and pose risks to decision-making. 


\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/hier_structure.png}
    \caption{An example of temporal hierarchical time series (HTS) structure for ten-minute frequency as the bottom level, half-hour and hour frequencies as aggregated levels of coarser granularity.}
    \label{fig:temporal_hts}
    \vspace{-5mm}
\end{figure}

%粗讲现在方法的问题， temporal hts then hts
Previous works on temporal hierarchy forecasting can be categorized into two types: vanilla forecasting methods for temporal HTS and multivariate HTS methods applied to temporal hierarchy. 
% Temporal hierarchy forecasting(\cite{thts_2017, theodosiou2021forecasting}) is less devoted compared to traditional multivariate hierarchy. 
Most temporal HTS methods~\cite{thts_2017, theodosiou2021forecasting} are statistical and theoretically explainable, but forecast performance is limited when applied to complex real-world datasets, implemented in the {\sc{thief}} package. 

The multivariate HTS methods typically follow a two-stage paradigm. In the first stage, base forecasts are generated independently for each time series in the hierarchy with statistical or deep learning models. In the second stage, base forecasts are adjusted via reconciliation to ensure coherence.

Most methods ignore the temporal hierarchical information among levels of different granularity in forecasting, one exception is COPDeepAR~\cite{rangapuram2023}, which leverages graph neural networks (GNNs) to extract structure information. 
% However, GNNs are too complex for the tree structure of hierarchy and may introduce noise information.
However, GNNs introduce noise connections between nodes in the tree structure and cause performance loss.
As for reconciliation, traditional statistical methods (e.g., MinT ~\cite{wickramasuriya2019optimal}) derive coherent forecasts relying on strong statistical assumptions. The end-to-end method~\cite{rangapuram2021end} ensures coherence without strong assumptions by using a closed-form projection. However, this may reduce the forecasting performance because the adjustment scale is sometimes either too large or small and could not adapt to node values.

In this paper, we propose a framework (GMP-AR) that efficiently utilizes information among granularity at different levels of temporal hierarchy to improve the forecast performance while maintaining coherence. In summary, our contributions are as follows:
\begin{itemize}
    \item 
    We propose a granularity message passing mechanism (GMP) to enrich the information of temporal input for each node and integrate the temporal hierarchical features among different granularity to generate base forecasts.
    This is the first method that employs the temporal hierarchical structure for forecasting tasks to the best of our knowledge.
    \item We provide an adaptive reconciliation method to produce coherent results without forecasting performance loss by utilizing the node-dependent weighted optimization target to precisely control the adjustment scale node by node. 
    \item We integrate our framework with an optimization module to solve real-world problems with task-based targets and realistic constraints.
    \item Experiments on real-world time series datasets demonstrate that our proposed approach achieves significant improvements over the state-of-the-art baselines and our framework combined with the optimization module has been deployed on the payment traffic management system in Alipay.
\end{itemize}



==> latex/method.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/architecture_v6.png}
    % \includegraphics[width=0.95\textwidth]{figures/architecture_v5.png}
    % \includegraphics[width=0.8\textwidth]{figures/architecture.png}
    \caption{The architecture of GMP-AR: the red dashed box is the granularity message passing component including the granularity input transformation module, temporal feature extractor, and two granularity feature fusion modules. This component generates the representation of nodes used to generate base forecasts and adaptive weights. The light green dashed box is the reconciliation module that produces the final results,
    including the adaptive reconciliation module for forecasting tasks and task-based optimization module to adapt to general real-world tasks.
    }
    \label{fig:architecture}
    \vspace{-5mm}
\end{figure*}

In this section, we introduce our framework (GMP-AR) that takes advantage of the message-passing to extract valid information among different granularity in the temporal hierarchy to improve forecasting performance and achieve adaptive reconciliation to maintain coherence.
% by leveraging neural networks to produce node-dependent weight.  
Finally, we integrate an efficient optimization module with our framework to solve real-world problems with task-based targets and realistic constraints. The overall architecture is shown in Fig.~\ref{fig:architecture}, which consists of three main components:
\begin{itemize}
    \item {\it Granularity message passing} module: This module leverages temporal hierarchy information between different granularity to generate base forecasts over the prediction horizon across all levels and adaptive weights;
    \item {\it Adaptive reconciliation} module: This module utilizes adaptive weights combined with projection reconciliation to produce node-dependent adjustment to maintain coherency in an end-to-end way;
    \item {\it `Plug-and-play' optimization} module: This module adapts to real-world problems with task-based targets and realistic constraints.
    % with task-based targets and realistic constraints. 
\end{itemize}


\subsection{Granularity Message Passing}
In this section, we introduce our granularity message-passing module that incorporates both temporal and granularity hierarchical information to generate the base forecasts and the weights for adaptive reconciliation. This module consists of four sub-modules: granularity input transformation, temporal feature extractor, and two granularity feature fusion modules.
% Child Granularity Feature Fusion, and Temporal and Hierarchical Granularity Feature Fusion.

\subsubsection{Granularity Input Transformation}
This module integrates the input information of different granularity in the hierarchy into temporal inputs by \textit{top-down proportion transformation} and \textit{child distribution modeling} as in Fig.~\ref{fig:input_trans}.
% \textit{Top-Down Proportions Transformation}

\textit{Top-Down Proportion Transformation.}
\begin{figure}
    \centering
    % \includegraphics[width=0.8\linewidth]{figures/input_transform.png}
    \includegraphics[width=0.9\linewidth]{figures/input_trans.png}
    \caption{The process of granularity input transformation: the orange cycle is the top-down proportion transformation module that produces the disaggregation proportions for child nodes, the red rectangle is the child distribution modeling module which extracts valid information of finer granularity for parent nodes; the blue box concatenate these processed inputs with normalized value and put them into temporal feature extractor to extract dynamic patterns.}
    \label{fig:input_trans}
    \vspace{-6mm}
\end{figure}
% This sub-module incorporates the structure information into the dynamic pattern extraction module by integrating the root node of coarse granularity into the leaf nodes of fine granularity at the bottom level to enhance temporal stability, which is based on the analysis that the seasonality of the top level is clearer and the evolutionary dynamic is smoother~\cite{demandforecast13, taieb2021hierarchical}.
Similar to the top-down proportion models in TDProb~\cite{das2022deep},
we transform the inputs $\{\by_1, \dots, \by_{\tau}\}$ as the fractions/proportions according to root time-series which is disaggregated
into its child time series as in Fig.~\ref{fig:input_trans}. The detail is as follows
% \begin{align}
%     a^{[p]}_{\tau +j} = \frac{y^{[p]}_{\tau  + j}}{y^{[1]}_{\tau}}, \quad \tau  \in \{1, 2, \dots, \lfloor\frac{T}{m}\rfloor \},
% \end{align}
\begin{align}
    a^{[k]}_{\tau,j} = \frac{y^{[k]}_{(\tau-1)n_k  + j}}{y^{[1]}_{\tau}}, \quad \tau  \in \left\{1, 2, \dots, \lfloor\frac{T}{m}\rfloor \right\},
\end{align}
where $a^{[k]}_{\tau,j}, 1\le j \le n_k$ is the fraction input at time $\tau $. Then we sort the fraction inputs from the root node to the current node to build the top-down proportion inputs $\boldsymbol{\alpha}_{\tau,j}^{[k]} = [a^{[2]}_{\tau, l_2}, \dots,  a^{[k]}_{\tau,j}],k\ge 2$, where $l_2$ means the node index at the second level on the path from the root to the current node, and {$l_i = \lceil l_{i+1} / \frac{n_{i+1}}{n_{i}} \rceil$}.  We use fraction inputs starting from the second level, as the fraction for the root level is always equal to $1$ and does not provide any meaningful information for the temporal extraction module.

The intuition behind this approach is as follows: 1) As pointed out in \cite{das2022deep}, the disaggregation proportions of nodes at the bottom level are more predictable compared to raw values of time series; 2) Incorporating the information of nodes at the top level with coarser granularity into the leaf nodes of finer granularity at the bottom level to enhance temporal stability, which is based on the analysis that the seasonality of the top level is clearer and the evolutionary dynamic is 'smoother' \cite{demandforecast13, taieb2021hierarchical}.

\textit{Child Distribution Modeling.}
% This sub-module integrates information from the finer granularity of child nodes to their parent at top levels, enhancing the framework's ability to adapt to the variation of dynamic patterns, such as sudden trend changes of special events. This is because the value aggregation relationship between the parent node and children nodes determines that changes in dynamic patterns at the finer granularity of children would influence the patterns of the coarser granularity of the parent.
This sub-module integrates the disaggregation proportion distribution of the child nodes with finer granularity into the temporal input of the parent node. This enriches the finer granularity information of the parent node, which help capture dynamic patterns more effectively for parent node with coarser granularity, improving the overall forecasting accuracy.

Our approach utilizes deep models to extract the distribution of child nodes' disaggregation proportions for each parent node.  Specifically, 
we assume that each node at the same level $k$ has the same number of children $m_k$, so the hierarchical structure is fixed for each upper level. Given the fixed structure, MLP~\cite{gardner1998artificial} is an efficient tool to extract features, 
% \begin{align}
%     b^{[p]}_{\tau  + j} = \text{MLP}([a^{[p+1]}_{\tau  +(j-1)m_{p+1}+l}: l \in \{1, 2, \dots, m_{p+1}\}]),
% \end{align}
% \begin{align}
%     b^{[k]}_{\tau, j} = \text{MLP}([a^{[k+1]}_{\tau,(j-1)n_{k+1}+l}: 1\le l \le n_{k+1}]),\,k < p,
% \end{align}
\begin{align}
    \mathbf{b}^{[k]}_{\tau, j} = \text{MLP}\left([a^{[k+1]}_{\tau,(j-1)m_{k}+l}: 1\le l \le m_{k}]\right),\,k < p,
\end{align}
where $\mathbf{b}^{[k]}_{\tau, j}$ represents the hidden features of child node's distribution for the parent node $y^{[k]}_{(\tau - 1) n_k  + j}$ and $\{a^{[k+1]}_{\tau,(j-1)m_{k} + l}: 1\le l \le m_{k}\}$ is the proportion input of its child set.  


\subsubsection{Temporal Feature Extraction.}
This module extracts temporal features for nodes at the same level (same granularity) as follows:
\begin{align*}
    h^{[k]}_{\tau,j} &= \text{UPDATE}^{[k]}\left(h^{[k]}_{\tau,j-1,}, [\boldsymbol{\alpha}^{[k]}_{\tau,j}, \mathbf{b}^{[k]}_{\tau,j}, \Bar{y}^{[k]}_{\tau,j}]; \theta^{[k]}\right), \\
    \mathbf{H}_{\tau } &= [h^{[1]}_{\tau,1 }, h^{[2]}_{\tau,1}, \dots, h^{[p]}_{\tau, m}] , 
\end{align*}
where $\boldsymbol{\alpha}^{[k]}_{\tau,j}$ is the top-down proportion inputs of node \textit{j} at level $k$ and time point $\tau $, $\mathbf{b}^{[k]}_{\tau,j}$ is the distribution feature of the child set, and $\Bar{y}^{[k]}_{\tau,j}$ is the scaled value of the sample at the same level over the whole past observations as follows:
% as the temporal scale in the same level as follows:
% \begin{align}
%     \Bar{y}^{[k]}_{\tau + j} = \frac{{y}^{[k]}_{\tau + j}}{\max\{y^{[k]}_{\tau - C + 1}, \dots, {y}^{[k]}_{\tau + n_k}\}},
% \end{align}
\begin{align}
    \Bar{y}^{[k]}_{\tau,j} = \frac{{y}^{[k]}_{(\tau-1)n_k + j}}{\max\{y^{[k]}_{1}, \dots, {y}^{[k]}_{\tau n_k}\}},\, 1\le j \le n_k.
\end{align}
 % $C$ is the global context length. 
Since the root node has no ancestors and the leaf nodes have no child, we remove $\boldsymbol{\alpha}_\tau^{[1]}$ for the coarsest granularity and $\mathbf{b}_{\tau,j}^{[p]}$ for the finest granularity. 
The module $\text{UPDATE}^{[k]}$ is a temporal pattern extraction function at level $k$, and $\theta^{[k]}$ is the parameters of the function. Any type of recurrent-type neural networks can be adopted as the temporal feature extraction
module, such as the RNN variants, TCN~\cite{bai2018empirical},  and
NBeats~\cite{oreshkin2019n}. In our experiments, we use GRU~\cite{chung2014empirical} for simplicity.
% without reducing observable performance.

It is worth emphasizing that temporal HTS differs from multivariate HTS in that different levels do not share the same temporal features. In multivariate HTS, all nodes are of the same temporal granularity and may have similar trends or seasonality.  However, in temporal HTS, nodes at different levels have different granularity and different context lengths. Nodes at the top levels,  which have coarser granularity, have smaller context lengths~\cite{rangapuram2023}.
In other words, different levels have their own dynamic patterns (trend, seasonality, etc.), which requires different specific parameters $\theta^{[k]}$ of temporal updating function for each level.

\subsubsection{Child Granularity Feature Fusion}
This module integrates temporal features from the finer granularity of child nodes to their parent at top levels, enhancing the framework's ability to adapt to the variation of dynamic patterns, such as sudden trend changes {due to some} special events, e.g., Double 11, black Friday. This because the value aggregation relationship between the parent node and child nodes determines the changes in dynamic patterns at the finer granularity would influence the ones at the coarser granularity.

Unlike directly modeling the disaggregation proportion distribution across child nodes, this module extracts valid temporal features from child nodes, which may have different contributions to their parent.  CNN and attention mechanism~\cite{vaswani2017attention} are effective tools to extract valid patterns from various features. However, we assume that all nodes at the same level have the same number of children, which indicates the tree structure at the same level is fixed.  For a fixed structure, CNN is more appropriate because it has lower computation cost (see Appendix E) and better performance as demonstrated in the ablation study (see Appendix F). The detail is as follows:
% and experiments conducted show performance is also better. :
\begin{align*}
    \hat{h}^{[k]}_{\tau, j} &= \text{Conv}^{[k]}\left([h^{[k+1]}_{\tau,(j-1)m_k + l}: 1 \le l \le m_{k}]\right)  \\
    &= \sum_{l=1}^{m_{k}} w^{[k]}_l h^{[k+1]}_{\tau, (j-1)m_k + l}\;,
\end{align*}
% \begin{align*}
%     \hat{h}^{[k]}_{\tau  + j} &= Conv^{[k]}([h^{[k+1]}_{\tau  + (j-1) n_{k+1} + s}]: s \in \{1, n_{k+1}\})  \\
%     &= \sum_{s=1}^{n_{k+1}} w^{[k]}_s h^{[k+1]}_{\tau  + (j-1) n_{k+1} + s},
% \end{align*}
where $\text{Conv}^{[k]}$ is the CNN kernel for level $k$, and the $w^{[k]}_l$ is the kernel weight of child $l$ at level $k$.
% , and $\hat{h}^{[k]}_{\tau, j}$ is the parent aggregation features.

\subsubsection{Temporal and Hierarchical Granularity Feature Fusion.}
This module integrates the temporal and hierarchical features among granularity for each node to enrich the dynamic and structure information of node representation, which is used to generate the base forecasts and the weights for adaptive reconciliation.

We adopt CNNs to extract valid information across the temporal and granularity hierarchy domains as follows:
\begin{align*}
    \Tilde{h}^{[k]}_{\tau, j} &= \text{Conv}(\hat{\mathbf{H}}^{[k]}_{\tau, j}; \theta), \\
    {\mathbf{\hat{H}}^{[k]}_{\tau, j}} 
    &= \begin{pmatrix}
        {h}^{[k]}_{\tau, 1} & \hat{h}^{[k]}_{\tau, 1}\\
        \vdots & \vdots \\
        {h}^{[k]}_{\tau,j} & \hat{h}^{[k]}_{\tau, j}
    \end{pmatrix},
\end{align*}
% \begin{align*}
%     \Tilde{h}^{[k]}_{\tau  + j} &= Conv2d(\Bar{\mathbf{H}}^{[k]}_{\tau  + j}; \theta), \\
%     {\mathbf{\Bar{H}}^{[k]}_{\tau  + j}} &= \begin{bmatrix}
%         h^{[k]}_{\tau  - C + j} & \hat{h}^{[k]}_{\tau  - C + j} \\\
%         \vdots & \vdots \\
%         h^{[k]}_{\tau  + j} & \hat{h}^{[k]}_{\tau  + j}
%     \end{bmatrix},
% \end{align*}
where all nodes share the same extraction parameters, $\Tilde{h}^{[k]}_{\tau, j}$ are used as inputs of MLPs (the module can be replaced with other neural layers, such as seq2seq~\cite{sutskever2014sequence}, transformers~\cite{vaswani2017attention}, and CNNs) to generate the base forecasts $\hat{\by}_\tau$ and reconciliation weights $\mathbf{w}$.
% in \mathbf{R}^{n\times n}

\subsection{Adaptive Reconciliation}
In this section, we introduce our adaptive reconciliation module by utilizing node-dependent weights that incorporate temporal and hierarchical information. These weights are used to control the adjustment scale node by node in reconciliation, improving the prediction performance and ensuring coherence.
% between different levels of the hierarchy.

Under the assumption that base forecasts are highly accurate, the closed-form projection reconciliation only minimizes the distance between the coherent result with the base forecast~\cite{rangapuram2021end}. However, the optimization target here is to minimize the mean distance among all nodes, which may result in a performance loss for several reasons. 
1) The scale of values among different nodes can be diverse, and mean distance minimization may cause a relatively large adjustment to the node with a small value, while only slight adjusting to the nodes with large values. Since the values at higher levels of the hierarchy have a coarser granularity that are larger than those at lower levels, the reconciliation mainly provides efficient adjustments to the upper level values. 
% 1) Considering the scale of values among different nodes can be diverse, inadequate adjustments would 
2) Since different nodes have distinct levels of forecasting accuracy,  the reconciliation adjustment scale should also be insignificant for nodes with high accuracy. In order to achieve adaptive adjustment node by node, node-dependent weights are imposed to the optimization target to resolve these issues as follows
\begin{equation}
    \begin{aligned}
    \label{eq:weight_recon}
     \Tilde{\by}_\tau & = \mathop{\arg\min}_{\by \in \mathbb{R}^n} \|\bw(\by - \hat{\by}_\tau) \|_2 \\
      % &= \mathop{\arg\min}_{\by \in \mathbb{R}^n} \frac{1}{2}{(\bw\by)}^{\mathsf{T}}{\bw\by} - {(\bw\hat{\by}_\tau)}^{\mathsf{T}}{\bw\by} \\
      \text{s.t.} &\quad \mathbf{A}{\by} = \mathbf{0},
    \end{aligned}
\end{equation}
where $\bw \in \mathbb{R}^{n \times n}$ is a diagonal matrix {with weights on the diagonal}. Then we apply the method of Lagrange multiplier to derive the closed-form solution (see the proof in Appendix A):
% Then we apply Lagrange relaxation to add an equation constraint to the target, 
% and let the partial gradient be equal to zero, then we derive the closed-form solution (the proof is shown in Appendix A):
% \begin{equation}\label{eq:analytic_sol}
%     \Tilde{\by}_{\tau } = M \hat{\by}_{\tau }
%      = (\mathbf{I} - \bw^{-1}\mathbf{A}^\mathsf{T}(\mathbf{A}\bw^{-1}\mathbf{A}^\mathsf{T})^{-1}\mathbf{A}) \hat{\by}_\tau
% \end{equation}
\begin{equation}\label{eq:analytic_sol}
    \Tilde{\by}_{\tau } = \mathbf{M} \hat{\by}_{\tau },
\end{equation}
where $\mathbf{M} = (\mathbf{I} - \tilde{\bw}^{-1}\mathbf{A}^\mathsf{T}(\mathbf{A}\tilde{\bw}^{-1}\mathbf{A}^\mathsf{T})^{-1}\mathbf{A}) \hat{\by}_\tau$, $\tilde{\bw} = {\bw^\mathsf{T}}{\bw}$.
% The weights can be hyperparameters for simple structures or some realistic tasks, or can even be generated by modeling for complex structures. Setting the hyperparameter approach is easy to implement to optimize and intuitive, but it is inflexible and the improvement in performance is limited. 

The node-dependent weights could be hyperparameters for simpler structures or realistic tasks, which is explainable and easy to implement.  However, it requires prior {domain} knowledge of each scenario to set {proper} weights, which causes inflexibility to new scenarios and the improvement of performance is limited.
Our framework utilizes temporal and hierarchical granularity to generate the node-dependent weights, which has superior performance improvement and adaptability than human settings as shown in Appendix F.
% which have been proven superior to the mean and predefined methods in Appendix.

\subsection{Task-based Optimization in Real-world Scenarios}
This module introduces an optimization module, which can be applied in our forecasting framework (GMP-AR) to solve real-world problems with task-based targets and realistic constraints. The detailed formulation is as follows:
% Previous works about temporal HTS and multivariate HTS most focus on the improvement of prediction accuracy, without considering the coherence constraint, making it unrealistic in many real-world tasks with specific limitations and practical targets, defined as follows:
\begin{equation}
    \label{eq:recon_task}
    \begin{aligned}
      &\mathcal{J}(\hat{\by}) = \mathop{\min}_{\by}{f(\hat{\by}, \by)}\\
    \text{s.t.}\quad 
    &\begin{cases}
    \mathbf{A}\by = \mathbf{0}, e_j = 0, \; j=1, \dots, n_{\text{eq}},\\
    g_i(\by, \hat{\by}) \le 0, \; i=1, \dots, n_{\text{ineq}}.
    \end{cases}
     \end{aligned}
\end{equation}
% \begin{equation}
%     \label{eq:recon_task}
%     \begin{aligned}
%       &\mathcal{J}(\hat{\by}) = \mathop{\arg\min}_{\by}{f(\hat{\by}, \by)}\\
%     \text{s.t.}\quad 
%     &\begin{cases}
%     \mathbf{A}\by = \mathbf{0}, e_j = 0, \; j=1, \dots, n_{\text{eq}},\\
%     g_i(\by, \hat{\by}) \le 0, \; i=1, \dots, n_{\text{ineq}}. 
%     \end{cases}
%      \end{aligned}
% \end{equation}
The target functional $f$ can take various forms of functions besides Euclidean distance (such as cosine similarity and $L^d$-norm ($d\ge 1$)){. The} $e_j$ terms represent task-based equality {constraints} other than coherence constraint{. The} $n_{\text{eq}}$ term is the number of equality constraints, the $g_i$ term is an inequality constraint, and $n_{\text{ineq}}$ term is the number of task-based inequality constraints. 
% In temporal HTS, the values of nodes in the history must keep invariant at reconciliation, and for inequality constraints, we may keep the predicted values positive.
As shown in Eq.~\eqref{eq:recon_task}, our task is transformed into an optimization task, where legacy methods such as L-BFGS or Powell~\cite{num_optim} can be applied.  Many useful optimization methods have been encapsulated in \textit{Scipy.optmize}, which is used in our experiment in Alipay with finance targets and supervised constraints.


==> latex/preliminary.tex <==
\section{Preliminaries}
\label{section: preliminaries}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/thier.png}
    \caption{The notation of each node in figure \ref{fig:temporal_hts} at time point $t^* =0$}
    \label{fig:temporal_hier}
\end{figure}
The temporal hierarchical time series can be denoted as a tree structure (see Figure \ref{fig:temporal_hts}) with linear aggregation constraints, expressed by aggregation matrix 
$\mathbf{S}\in \mathbb{R}^{n \times m}$
($m$ is the number of bottom-level nodes, and $n$ is the total number of nodes).

{{\color{red} to be revised: }Given a time series denoted by $\{y_t; t\in \{1,2,\dots,T\}\}$ of the most precise sampling frequency.} We fix a \textit{p-level} aggregated temporal hierarchical structure to define the notation.
The number of nodes in each level can be presented as $\{n_k: k  \in \{1, 2, \dots, p\}\}$, where $n_1 = 1$, and $n_p := m$ where \textit{m} is the number of leaves in the temporal structure. Take Figure as an example, the nodes are as $\{1, 2, 6\}$. And the time points of aggregated level \textit{k} time series can be presented as:

\begin{equation}
    y_{t^*+j}^{[k]} = \sum_{t=t^*m+(j-1)m_k} ^ {t^*m+jm_k - 1} y_t, \quad j \in \{1, 2, \dots, n_k\}
\end{equation}

where j means the index in level k in one temporal structure, and the $t^*$ means the observation index of the
most aggregated series (i.e., root level), in order to use a
common index for all levels. And the $m_k = \frac{m}{n_k}$, which means the number of leave aggregated to generate the time point of \textit{kth} level, which also means the children number on the level. 

In the temporal hierarchical structure, the leaf nodes are called the \textit{bottom-level} series $\by^{[p]}_{t}\in \mathbb{R}^{m}$, and those of the remaining nodes are termed the \textit{upper-levels} series $\{\by^{[1]}_{t}, \dots, \by^{[p-1]}_{t} \}$, the number of nodes of upper levels is $r=\sum_{i=1}^{p-1} n_i$.
Obviously, the total number of nodes $n=r+m$, and $\by_{t} :=[y^{[1]}_{t}, \by^{[2]}_{t}, \dots, \by^{[p]}_{t}]^{\mathsf{T}} \in  \mathbb{R}^{n} $ contains observations at time $t^*$ for all levels, which satisfies  
\begin{equation}
\label{eq_sum}
\by_{t^*}=\bS \by^{[p]}_{t^*},
\end{equation}
% at time step $t$.
where $\bS\in \{0,1\}^{n \times m}$ is an aggregation matrix. 

Taking the temporal hierarchical structure in Figure~\ref{fig:hier_timeseries} as an example, the aggregation matrix 
% \replace{takes}
{is in} the form:
% as in Eq.~\eqref{eq:hts_matrix}

\begin{equation*} %\label{eq:hts_matrix}
    \bS = 
    \begin{bmatrix}
        \bS_{\text{sum}}\\
        \mathbf{I}_6
    \end{bmatrix}
    \begin{bmatrix}
    \begin{array}{cccccc}
        1 & 1 & 1 &1 & 1 &1 \\
        1 & 1 & 1 &0 &0 &0\\
        0 & 0 & 0 &1 &1 & 1\\
        % \hline \\
        \hdotsfor{6}\\
        % & & & & \\
        & & \mathbf{I}_6 & &\\
        % & & & &
     \end{array} 
     \end{bmatrix}
     % \right]
     ,
\end{equation*}
% Figure ~\ref{fig:hier_timeseries}, 
and the total number of nodes in the hierarchy is $n=1+2+6$.  At each time step $t^*$, 
% \begin{equation*}
%     \begin{aligned}
%         \mathbf{u}_{t}&=[y_{A,t},y_{B,t},y_{C,t}] \in \mathbb{R}^{3}, \\
%         \mathbf{b}_{t}&=[y_{D,t},y_{E,t},y_{F,t},y_{G,t},y_{H,t}] \in \mathbb{R}^{5},\\
%         y_{A,t}&=y_{B,t}+y_{C,t}=y_{D,t}+y_{E,t}+y_{F,t}+y_{G,t}+y_{H,t}.
%     \end{aligned}
% \end{equation*}
% $ and $\mathbf{b}_{t}=[y_{D,t},y_{E,t},y_{F,t},y_{G,t},y_{H,t}] \in \mathbb{R}^{5}$, $y_{A,t}=y_{B,t}+y_{C,t}=y_{D,t}+y_{E,t}+y_{F,t}+y_{G,t}+y_{H,t} $.
% , and the aggregation matrix $\bS\in \{0,1\}^{8 \times 5}$.

The coherence constraint of Eq.~\eqref{eq_sum} can be represented as ~\cite{rangapuram2021end}
\begin{equation}
\label{eq:coherent_co}
\mathbf{A}\by_{t}=\mathbf{0},
\end{equation}
where $\mathbf{A}:=[\mathbf{I}_{r}|-\bS_{sum}] \in \{0,1\}^{r \times n}$, $\mathbf{0}$ is an $r$-vector of zeros, and $\mathbf{I}_{r}$ is the $r \times r $ identity matrix.  %We will use this formula as the coherence constraint for the rest of the paper.



==> latex/rebuttal.tex <==
% \section{rebuttal}
We thank all the reviewers for the questions. As suggested, we will update the paper to include further explanations. Below we answer each question for every reviewer. 
\subsection{To Reviewer \#2}
\begin{itemize}
    \item Weakness 1: 
    \begin{itemize}
        \item We provide an example in Figure 2, we will follow your advice to point it out later. The above notations and statements are consistent with previous works, e.g., \cite{thts_2017}.
        \item For notation $\bS$ (Weakness 1.2) and $\mathbf{A}$ (Weakness 1.3), they are both standard matrix notations to describe aggregation constraints in hierarchy structure \cite{SLOTH_2023, thts_2017}.
        \item see above
        \item Thanks for your advice, we'll fix it in the final version. 
        % \item As shown in the first graph on page 4 in Section \textbf{Child Granularity Feature Fusion}, we introduce valid patterns that include sudden trend changes due to some special events, e.g., Double 11, black Friday.
        \item {In the first graph on page 4 of the ``Child Granularity Feature Fusion" section, we introduce patterns that accurately capture sudden trend changes caused by specific events such as Double 11 and Black Friday.}
        \item The general equality constraints notation $e_j$ is consistent with reference \cite{amos2017optnet, SLOTH_2023}, and we provided an example in Equation (10), we’ll point it out in the final version of the paper.
        % We will illustrate this in the CRV for the readers' convenience.
        \item Figure 6 shows that our model {equipped} with optimization module gets a trend accuracy loss of 0.28\% ({0.7325 vs. 0.7297}). There is nearly no performance loss compared to the improvement in MAPE by 3.8\% {as indicated in the caption}.
    \end{itemize} 
    \item Weakness 2: {The experiment in the section (Alipay Payment Traffic Management) are based on the real Alipay fund traffic data, and the results demonstrate the outstanding performance and applicability of our method.}
\end{itemize}


\subsection{To Reviewer \#3}
\begin{itemize}
    \item Weakness 1: The notion that GNNs introduce noise stems from the observation made by \cite{SLOTH_2023} that GNNs connect unrelated nodes within hierarchical structures, leading to the propagation of noisy information. Our GMP module integrates information between nodes with aggregation relationships along the path from root to leaf, effectively preventing the introduction of noise.
    \item Weakness 2: Thanks, we will update it in final version.
    \item Weakness 3: Thanks for your advice. The complexity of our GMP module is $\mathbf{O(NlogN)}$. We provide running time analysis for all methods in \textbf{Appendix E}, our method has lower complexity and time cost {than other methods}.
    \item Question 1: It means that the same adjustment can result in varying accuracy losses for different nodes. For instance, consider two child nodes of a parent node with values of 10000 and 100. If an adjustment of 50 is applied, it will induce an accuracy change of only 0.5\% for the node with value 10000, but a significant 50\% accuracy change for the node with value 100.
    \item Question 2: Similar to question 1, if the adjustment is 1, it is negligible for node 10000, because it only causes 0.01\% accuracy adjustment.
    \item Question 3: It means it is easier to predict the fraction of the bottom nodes allocated from the root node compared to the bottom values. {This is due to that the fraction exhibits greater stability than the absolute value.}   
\end{itemize}

\subsection{To Reviewer \#4}
\begin{itemize}
    \item Weakness 1: We have evaluated our method on 3 publicly available time series datasets in the section \textbf{Result Analysis}, and we also present the detailed analysis in \textbf{Appendix D} and ablation study in \textbf{Appendix F}. 
    \item Weakness 2: We provide the pros and cons of vanilla forecasting methods and multivariate HTS methods in the \textbf{Related Work} section. Besides, we present results for different types of methods in \textbf{Table 1} and introduce it in the first paragraph in \textbf{Result Analysis}.
    \item Weakness 3 (Question 2): {We appreciate your valuable feedback. We have already provided an illustrative example in the first graph of the \textbf{Introduction} demonstrating that inconsistencies between short-term and long-term forecasts can lead to either unmet commodity demand or excessive inventory costs in retail operations. We will strive to provide an even more comprehensive assessment of this issue in the final version of our paper.}
    \item Question 1: As shown in section \textbf{Method}, our GMP-AR framework firstly utilizes the temporal structure information to improve forecast performance, and achieves node-dependent adaptive reconciliation to {satisfy} coherency.
\end{itemize}


\subsection{To Reviewer \#5}
\begin{itemize}
    \item Weakness 1: The time series at the bottom level (the finest granularity) is consistent with real data (Traffic, Electricity, Exchange Rate), and the values of top levels are aggregated from real data. We have tried different aggregation settings to validate the scalability in \textbf{Table 2}.  
    \item Weakness 2: Thank you for your advice, we have introduced an example in \textbf{Alipay Payment Traffic Management}, and we will provide more details in the final version. The results generated from the optimization module would satisfy constraints first, so no matter whether the objective is easy or hard to optimize, the constraint will be always valid.
    \item Weakness 3: Thank you for your advice. We will provide other metrics (MSE, b-MAPE) in the final version.
\end{itemize}

==> latex/related_work.tex <==

\subsection{Temporary Hierarchical Structure}
Given a time series with ${y_0, y_1, ..., y_t}$ with a fixed sampling frequency called base frequency, which is the finest granularity. The time series of the coarsest granularity is aggregated by non-overlapping and regularly sampled values $y_t$ as equation {\color{red} ??} shows. As in Fig. \ref{fig:temporal_hts}, the base frequency is one quarter, it aggregates the time series to a semi-annual value with two quarter values and yearly frequency with two semester values.

Most well-known hierarchical structures in time series forecasting field are tree structure in the cross-sectional of a multivariate time series, in which each node represents an individual time series. Unlikely, the temporal hierarchical structure is constructed by a univariate time series that sampled with different frequencies, and the nodes at the same level in the tree represent values sampled in time intervals of equal length with different start points. The higher level corresponds to coarser granularity or lower frequency, and the root level corresponds to the coarsest granularity. The number of children of the parent node in the temporal hierarchy is determined
by the coarseness of aggregation frequency. For example, in the
case of quarterly sampled data, if the top-level frequency is one year, then the number of children nodes is four.


\subsection{Time Series Forecasting}
Existing time series forecasting methods can be roughly grouped into two categories: classical statistical models and deep learning-based models. Statistical time series models are widely used in both industrial and research areas with  interpretability and theoretical guarantee (ARIMA, ETS). Deep learning-based models are popular due to ground-breaking performance, these methods mainly depend on the RNN and their variants to model the dynamic pattern with deep neural networks.


\subsection{Hierarchical Time Series Forecasting}
Multivariate time series forecasting with complex hierarchical
structures has been applied in various real-world problems. The critical challenge in hierarchical forecasting tasks
lies in producing accurate prediction results while satisfying
aggregation (coherence) constraints as Eq shows. 
Traditional approaches try to generate the base forecast of the pre-specified level first, then the reconciliation method is applied to satisfy the coherence. Traditional methods use statistical methods like ARIMA, ETS to generate the base forecasts. But due to the superior performance of deep neural networks, deep-learning forecasting methods are applied to base forecasts such as DeepAR, DeepVAR.
As for the reconciliation method, the traditional depends on one level of the forecast, e.g. Bottom-Up mechanism \cite{gross1990disaggregation} which aggregates the base forecast from the bottom level to high levels, Top-Down mechanism \cite{athanasopoulos2009hierarchical} disaggregated the top level forecast to bottom-levels, Middle-out mechanism \cite{athanasopoulos2017forecasting} produce the forecasts  at a middle level of the hierarchy, followed by aggregations for the higher levels and disaggregations for the lower ones. But these methods only use single-level forecasts to conduct reconciliation, the forecasts of other levels are ignored. Recently researchers proposed the MinT method which leverages all level information of base distribution forecasts to generate coherent results. And HierE2E proposes a closed-form projection  method to achieve an end-to-end reconciliation.
However, this method has the following limitations: 1) the structure information in the hierarchy is not utilized efficiently to produce the base forecasts; 2) the closed-form projection produce unreasonable forecast results without value constraint.



% \subsection{Reconciliation}



